Bounding Box Priors for Cell Detection with Point Annotations

The size of an individual cell type, such as a red blood cell, does not vary much among humans. We use this knowledge as a prior for classifying and detecting cells in images with only a few ground truth bounding box annotations, while most of the cells are annotated with points. This setting leads to weakly semi-supervised learning. We propose replacing points with either stochastic (ST) boxes or bounding box predictions during the training process. The proposed "mean-IOU" ST box maximizes the overlap with all the boxes belonging to the sample space with a class-specific approximated prior probability distribution of bounding boxes. Our method trains with both box- and point-labelled images in conjunction, unlike the existing methods, which train first with box- and then point-labelled images. In the most challenging setting, when only 5% images are box-labelled, quantitative experiments on a urine dataset show that our one-stage method outperforms two-stage methods by 5.56 mAP. Furthermore, we suggest an approach that partially answers "how many box-labelled annotations are necessary?" before training a machine learning model.

==> plot_pdf.tex <==
\pgfplotsset{
compat=1.7,
legend image code/.code={
\draw[mark repeat=2,mark phase=2]
plot coordinates {
(0cm,0cm)
(0.15cm,0cm)        %% default is (0.3cm,0cm)
(0.2cm,0cm)         %% default is (0.6cm,0cm)
};%
every axis legend/.append style={
at={(8,8)},
anchor=north,
inner sep=0pt, outer sep=0pt}
}
}

\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.49\linewidth}
    \pgfplotstableread[col sep=comma]{data/USD_pdf.csv}\loadedtable
    \begin{tikzpicture}[font=\footnotesize,inner sep=2pt, outer sep=0pt]
      \begin{axis}[
        scale = 0.5,
        title = {(a) USD},
        table/col sep=comma,
        axis lines = left,
        xmin=2.5, xmax=7, ymin=0, ymax=2.5,
        xtick={3,4,5,6},
        no markers,
        xlabel = $\log$(width), ylabel = pdf,
        yticklabels={,,},
        cycle list name=exotic,
        %colormap/violet,
        legend entries = {eryth,leuko,epith,epithn,mycete,cryst,cast},
        legend style={font=\footnotesize,draw=none,inner sep=0pt, outer sep=0pt,at={(1,1)},
anchor=north east},
        legend cell align={left},
      ]
      \addplot +table[x=xi, y=eryth]{\loadedtable};
      \addplot +table[x=xi, y=leuko]{\loadedtable};
      \addplot +table[x=xi, y=epith]{\loadedtable};
      \addplot +table[x=xi, y=epithn]{\loadedtable};
      \addplot +table[x=xi, y=mycete]{\loadedtable};
      \addplot +table[x=xi, y=cryst]{\loadedtable};
      \addplot +table[x=xi, y=cast]{\loadedtable};
      \end{axis}
    \end{tikzpicture}
    \end{minipage}
    \begin{minipage}[b]{0.49\linewidth}
    \pgfplotstableread[col sep=comma]{data/BCCD_pdf.csv}\loadedtable
    \begin{tikzpicture}[font=\footnotesize,inner sep=2pt, outer sep=0pt]
      \begin{axis}[
        scale = 0.5,
        title = {(b) BCCD},
        table/col sep=comma,
        axis lines = left,
        xmin=2.5, xmax=7, ymin=0, ymax=3.5,
        xtick={3,4,5,6},
        yticklabels={,,},
        cycle list name=exotic,
        no marks,
        xlabel = $\log$(width), ylabel = {},
        legend entries = {platelets, rbc, wbc},
        legend style={font=\footnotesize,draw=none,inner sep=0pt, outer sep=0pt,at={(1.1,1)},
anchor=north east},
        legend cell align={left},
      ]
      \addplot table[x=xi, y=Platelets]{\loadedtable};
      \addplot table[x=xi, y=RBC]{\loadedtable};
      \addplot table[x=xi, y=WBC]{\loadedtable};
      \end{axis}
    \end{tikzpicture}
    \end{minipage}
    \caption{Approximated prior probability density functions (pdf) of the width of bounding boxes of all seven classes in the USD and all three classes in the BCCD cell datasets.}
    \label{fig:pdf}
\end{figure}

